Benchmarking Zero-Shot Robustness of Multimodal Foundation Models: A Pilot Study

Pre-training image representations from the raw text about images enables zero-shot vision transfer to downstream tasks. Through pre-training on millions of samples collected from the internet, multimodal foundation models, such as CLIP, produce state-of-the-art zero-shot results that often reach competitiveness with fully supervised methods without the need for task-specific training. Besides the encouraging performance on classification accuracy, it is reported that these models close the robustness gap by matching the performance of supervised models trained on ImageNet under natural distribution shift. Because robustness is critical to real-world applications, especially safety-critical ones, in this paper, we present a comprehensive evaluation based on a large-scale robustness benchmark covering 7 natural, 3 synthetic distribution shifts, and 11 adversarial attacks. We use CLIP as a pilot study. We show that CLIP leads to a significant robustness drop compared to supervised ImageNet models on our benchmark, especially under synthetic distribution shift and adversarial attacks. Furthermore, data overlap analysis suggests that the observed robustness under natural distribution shifts could be attributed, at least in part, to data overlap. In summary, our evaluation shows a comprehensive evaluation of robustness is necessary; and there is a significant need to improve the robustness of zero-shot multimodal models.

==> figs/advin.tex <==
\begin{figure*}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{figs/adv_robustness_imgNet.pdf}
    \vspace{-0.05in}
    \caption{\focus{\small Average model accuracies under adversarial attacks on the ImageNet. \yangyi{update linear fit}}}
    \label{fig:advin}
\end{figure*}

==> figs/alladv.tex <==
\begin{figure*}
\centering
\subcaptionbox{{\small Average model accuracies under common adversarial attacks on ImageNet and CIFAR-10.}\label{fig:alladva}}{\includegraphics[width=0.5\textwidth]{figs/all_adv_robustness.pdf}}%
% \hspace{0.05in}
\subcaptionbox{{\small Average model accuracies under typographic attacks on ImageNet-T and CIFAR-10-T.}\label{fig:alladvb}}{\includegraphics[width=0.5\textwidth]{figs/typographic_attack.pdf}}%
\caption{{\small Results on adversarial attacks.}}
    \label{fig:alladv}
\end{figure*}

==> figs/alldist.tex <==
\comm{
\begin{figure*}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{figs/general_robustness.pdf}
    \vspace{-0.05in}
    \caption{\focus{\small Average model accuracies on the seven natural distribution shifts.}}
    \label{fig:natural}
\end{figure*}
\begin{figure*}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{figs/imgnetC.pdf}
    \vspace{-0.05in}
    \caption{\focus{\small Average model accuracies (Corruptions Averaged) on ImageNet-C.}}
    \label{fig:inc}
\end{figure*}
}

\begin{figure*}
\centering
\subcaptionbox{{\small Average model accuracies on the seven natural distribution shifts.}\label{fig:alldista}}{\includegraphics[width=0.5\textwidth]{figs/general_robustness.pdf}}%
% \hspace{0.05in}
\subcaptionbox{{\small Average model accuracies on ImageNet-C and Stylized ImageNet (top-1, \%)}\label{fig:alldistb}}{\includegraphics[width=0.5\textwidth]{figs/imgnetC.pdf}}%
\caption{{\small Results on distribution shifts.}}
    \label{fig:alldist}
\end{figure*}

==> figs/dataoverlap.tex <==
\begin{figure*}[h]
    \centering
    \includegraphics[width=0.9\textwidth]{figs/datasets.pdf}
    \vspace{-0.05in}
    \caption{{\small Data overlap examples. We use Google Images to find the similar or same images in ImageNetV2.}}
    \label{fig:dataoverlap}
\end{figure*}

==> figs/dataoverlapmore.tex <==
\begin{figure*}[h]
    \centering
    \includegraphics[width=0.9\textwidth]{figs/datasets.pdf}
    \vspace{-0.05in}
    \caption{{ More data overlap examples between the pre-training data of CLIP and natural distribution shifts. We randomly sample several images from each natural distribution shift dataset, and use Google Images API to find the similar or same images. Even though the pre-training data of CLIP has not been released yet, we are able to identify the potential data contamination issue.}}
    \label{fig:dataoverlapmore}
\end{figure*}

==> figs/sin.tex <==

\begin{figure*}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{figs/stylized_imagenet.pdf}
    \vspace{-0.05in}
    \caption{{\small Model accuracies on Stylized ImageNet.}}
    \label{fig:sin}
\end{figure*}

==> tabs/googleimage.tex <==
\begin{table*}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lll@{}}
Dataset                          & Google Images (url)                                                                                                                      &  \\
\multirow{2}{*}{ImageNet-Sketch} & https://thumbs.dreamstime.com/b/hand-drawn-banana-sketch-isolated-white-background-banana-fruit-sketch-vector-illustration-209862105.jpg &  \\
                                 &                                                                                                                                          &  \\
\multirow{2}{*}{ImageNet-A}      & https://live.staticflickr.com/3842/33131828552\_3a72d700d8\_n.jpg                                                                        &  \\
                                 &                                                                                                                                          & 
\end{tabular}%
}
\caption{Similar images from Google Images.}
\label{tab:googleexample}
\end{table*}

==> tabs/imagenet-P-mfr.tex <==

\begin{table}[]
\resizebox{0.95\linewidth}{!}{

\begin{tabular}{llccccccccccc}
\multicolumn{2}{l}{\textbf{}}                       & \multicolumn{1}{r}{\textbf{}} & \multicolumn{2}{c}{\textbf{Noise}}          & \multicolumn{2}{c}{\textbf{Blur}}           & \multicolumn{2}{c}{\textbf{Weather}}        & \multicolumn{4}{c}{\textbf{Digital}}                                                      \\ \hline
\multicolumn{2}{l}{\textbf{Model}}                  & \textbf{mFR}                  & \textbf{Gaussion}    & \textbf{Shot}        & \textbf{Motion}      & \textbf{Zoom}        & \textbf{Snow}        & \textbf{Bright}      & \textbf{Translate}   & \textbf{Rorate}      & \textbf{Tilt}        & \textbf{Scale}       \\ \hline
\multirow{5}{*}{ResNet50}   & Standard         & \best 57.90                         &\best 59.00                & \best58.00                & \best64.00                &\best 72.00                & \best63.00                & \best62.00                & \best44.00                & \best52.00                & \best57.00                & \best48.00                \\
                                 & CLIP             & 113.69                        & 99.59                & 93.34                & 129.19               & 147.51               & 118.32               & 148.67               & 99.13                & 102.11               & 129.09               & 70.00                \\
                                 & CLIP-Sinlge      & 118.58                        & 106.34               & 98.59                & 133.10               & 152.58               & 121.63               & 156.79               & 102.63               & 106.71               & 134.78               & 72.67                \\
                                 & CLIP-Auto-Single \ours & 114.94                        & 101.22               & 94.55                & 130.30               & 148.82               & 119.62               & 149.53               & 99.54                & 103.77               & 130.81               & 71.26                \\
                                 & CLIP-Auto \ours       & \secbest 110.62                        &\secbest  95.18                & \secbest 90.29                & \secbest 125.63               & \secbest 143.40               & \secbest 117.65               & \secbest 143.62               & \secbest 96.41                & \secbest 99.66                & \secbest 125.83               & \secbest  68.55                \\ \hline
\multirow{5}{*}{ResNet101}  & Standard         & \best  53.02                         & \best55.10                & \best51.70                &\best 53.77                & \best63.25                & \best58.80                &\best 57.32                & \best42.25                & \best48.96                &\best 53.65                & \best45.35                \\
                                 & CLIP             & 98.91                         & 82.82                & 78.80                & 108.99               & 129.43               & 104.07               & 129.08               & 89.22                & 90.17                & 113.72               & 62.79                \\
                                 & CLIP-Sinlge      & 103.12                        & 87.27                & 82.50                & 111.65               & 133.45               & 107.40               & 136.26               & 92.95                & 94.29                & 119.50               & 65.89                \\
                                 & CLIP-Auto-Single \ours& 99.99                         & 84.27                & 80.35                & 109.69               & 130.37               & 105.26               & 131.08               & 89.20                & 90.74                & 115.39               & 63.57                \\
                                 & CLIP-Auto   \ours     &\secbest  97.23                         &\secbest  81.51                &\secbest  77.38                & \secbest 108.10               & \secbest 127.41               & \secbest 103.15               & \secbest 127.22               &\secbest  86.67                &\secbest  88.12                & \secbest 110.71               &\secbest  62.08                \\ \hline
\multirow{5}{*}{ViT-B/32}   & Standard         & \best 35.26                         & \best 28.23                & \best27.76                &\best 32.70                & \best46.46                & \best34.86                &\best 56.44                & \best35.79                & \best45.69                & \best43.05                & \best44.54                \\
                                 & CLIP             & 74.53                         & 64.56                & 58.40                & 66.85                & 93.94                & 71.13                & 94.87                & 67.26                & 76.61                & 88.34                & 63.35                \\
                                 & CLIP-Sinlge      & 77.33                         & 66.85                & 61.33                & 69.24                & 98.30                & 73.72                & 98.20                & 69.14                & 79.60                & 91.99                & 64.95                \\
                                 & CLIP-Auto-Single \ours & 76.95                         & 65.59                & 59.58                & 70.17                & 98.38                & 74.44                & 97.77                & 67.93                & 78.89                & 91.45                & 65.24                \\
                                 & CLIP-Auto   \ours     & \secbest 72.14                         & \secbest 61.17                & \secbest56.20                & \secbest65.02                & \secbest92.26                & \secbest70.00                & \secbest90.61                & \secbest64.49                & \secbest74.81                & \secbest85.04                & \secbest 61.81                \\ \hline
\multirow{4}{*}{ResNet50x4} & CLIP             & \secbest 90.07                         &\best  71.05                &\best  68.37                &\secbest 107.20               &\secbest  125.19               & \best101.92               & \secbest 117.69               & \secbest 72.61                & \secbest79.64                & \secbest 101.59               & \secbest 55.47                \\
                                 & CLIP-Sinlge      & 96.72                         & 77.25                & 74.38                & 112.69               & 131.72               & 107.87               & 125.69               & 79.22                & 87.48                & 110.65               & 60.23                \\
                                 & CLIP-Auto-Single \ours & 93.05                         & 74.15                & 70.87                & 109.88               & 127.78               & 104.95               & 121.96               & 75.14                & 82.75                & 105.86               & 57.19                \\
                                 & CLIP-Auto    \ours    & \best  89.42                         & \secbest 71.15                & \secbest 68.57                & \best 106.49               & \best 122.51               & \secbest  102.64               & \best 116.73               & \best 72.52                & \best 78.80                & \best  99.77                & \best  55.03                \\ \hline
                                 &                  &                               &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      \\
                                 &                  &                               &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      \\
                                 &                  & \multicolumn{1}{l}{}          & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}
\end{tabular}

}
\caption{{\small mFR on ImageNet-P.}}
\label{tab:imgnetPmfr}
\end{table}




\comm{
\begin{table}[]
% \resizebox{0.95\linewidth}{!}{
\begin{subtable}[t]{0.48\textwidth}
\begin{tabular}{llccccccccccc}
\multicolumn{2}{l}{\textbf{}}                       & \multicolumn{1}{r}{\textbf{}} & \multicolumn{2}{c}{\textbf{Noise}}          & \multicolumn{2}{c}{\textbf{Blur}}           & \multicolumn{2}{c}{\textbf{Weather}}        & \multicolumn{4}{c}{\textbf{Digital}}                                                      \\ \hline
\multicolumn{2}{l}{\textbf{Model}}                  & \textbf{mFR}                  & \textbf{Gaussion}    & \textbf{Shot}        & \textbf{Motion}      & \textbf{Zoom}        & \textbf{Snow}        & \textbf{Bright}      & \textbf{Translate}   & \textbf{Rorate}      & \textbf{Tilt}        & \textbf{Scale}       \\ \hline
\multirow{5}{*}{ResNet50}   & Standard         & \best 57.90                         &\best 59.00                & \best58.00                & \best64.00                &\best 72.00                & \best63.00                & \best62.00                & \best44.00                & \best52.00                & \best57.00                & \best48.00                \\
                                 & CLIP             & 113.69                        & 99.59                & 93.34                & 129.19               & 147.51               & 118.32               & 148.67               & 99.13                & 102.11               & 129.09               & 70.00                \\
                                 & CLIP-Sinlge      & 118.58                        & 106.34               & 98.59                & 133.10               & 152.58               & 121.63               & 156.79               & 102.63               & 106.71               & 134.78               & 72.67                \\
                                 & CLIP-Auto-Single \ours & 114.94                        & 101.22               & 94.55                & 130.30               & 148.82               & 119.62               & 149.53               & 99.54                & 103.77               & 130.81               & 71.26                \\
                                 & CLIP-Auto  \ours       & \secbest 110.62                        &\secbest  95.18                & \secbest 90.29                & \secbest 125.63               & \secbest 143.40               & \secbest 117.65               & \secbest 143.62               & \secbest 96.41                & \secbest 99.66                & \secbest 125.83               & \secbest  68.55                \\ \hline
\multirow{5}{*}{ResNet101}  & Standard         & \best  53.02                         & \best55.10                & \best51.70                &\best 53.77                & \best63.25                & \best58.80                &\best 57.32                & \best42.25                & \best48.96                &\best 53.65                & \best45.35                \\
                                 & CLIP             & 98.91                         & 82.82                & 78.80                & 108.99               & 129.43               & 104.07               & 129.08               & 89.22                & 90.17                & 113.72               & 62.79                \\
                                 & CLIP-Sinlge      & 103.12                        & 87.27                & 82.50                & 111.65               & 133.45               & 107.40               & 136.26               & 92.95                & 94.29                & 119.50               & 65.89                \\
                                 & CLIP-Auto-Single \ours & 99.99                         & 84.27                & 80.35                & 109.69               & 130.37               & 105.26               & 131.08               & 89.20                & 90.74                & 115.39               & 63.57                \\
                                 & CLIP-Auto  \ours      &\secbest  97.23                         &\secbest  81.51                &\secbest  77.38                & \secbest 108.10               & \secbest 127.41               & \secbest 103.15               & \secbest 127.22               &\secbest  86.67                &\secbest  88.12                & \secbest 110.71               &\secbest  62.08                \\ \hline
\multirow{5}{*}{ViT-B/32}   & Standard         & \best 35.26                         & \best 28.23                & \best27.76                &\best 32.70                & \best46.46                & \best34.86                &\best 56.44                & \best35.79                & \best45.69                & \best43.05                & \best44.54                \\
                                 & CLIP             & 74.53                         & 64.56                & 58.40                & 66.85                & 93.94                & 71.13                & 94.87                & 67.26                & 76.61                & 88.34                & 63.35                \\
                                 & CLIP-Sinlge      & 77.33                         & 66.85                & 61.33                & 69.24                & 98.30                & 73.72                & 98.20                & 69.14                & 79.60                & 91.99                & 64.95                \\
                                 & CLIP-Auto-Single \ours & 76.95                         & 65.59                & 59.58                & 70.17                & 98.38                & 74.44                & 97.77                & 67.93                & 78.89                & 91.45                & 65.24                \\
                                 & CLIP-Auto \ours       & \secbest 72.14                         & \secbest 61.17                & \secbest56.20                & \secbest65.02                & \secbest92.26                & \secbest70.00                & \secbest90.61                & \secbest64.49                & \secbest74.81                & \secbest85.04                & \secbest 61.81                \\ \hline
\multirow{4}{*}{ResNet50x4} & CLIP             & \secbest 90.07                         &\best  71.05                &\best  68.37                &\secbest 107.20               &\secbest  125.19               & \best101.92               & \secbest 117.69               & \secbest 72.61                & \secbest79.64                & \secbest 101.59               & \secbest 55.47                \\
                                 & CLIP-Sinlge      & 96.72                         & 77.25                & 74.38                & 112.69               & 131.72               & 107.87               & 125.69               & 79.22                & 87.48                & 110.65               & 60.23                \\
                                 & CLIP-Auto-Single \ours & 93.05                         & 74.15                & 70.87                & 109.88               & 127.78               & 104.95               & 121.96               & 75.14                & 82.75                & 105.86               & 57.19                \\
                                 & CLIP-Auto  \ours      & \best  89.42                         & \secbest 71.15                & \secbest 68.57                & \best 106.49               & \best 122.51               & \secbest  102.64               & \best 116.73               & \best 72.52                & \best 78.80                & \best  99.77                & \best  55.03                \\ \hline
                                 &                  &                               &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      \\
                                 &                  &                               &                      &                      &                      &                      &                      &                      &                      &                      &                      &                      \\
                                 &                  & \multicolumn{1}{l}{}          & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}
\end{tabular}
\caption{{\small mFR.}}
\label{tab:imgnetPmfr}
\end{subtable}

% \begin{table}[]
% \resizebox{0.95\linewidth}{!}{
\begin{subtable}
\begin{tabular}{llccccccccccc}
\multicolumn{2}{c}{\textbf{}}                       & \textbf{}     & \multicolumn{2}{c}{\textbf{Noise}} & \multicolumn{2}{c}{\textbf{Blur}} & \multicolumn{2}{c}{\textbf{Weather}} & \multicolumn{4}{c}{\textbf{Digital}}                                  \\ \hline
\multicolumn{2}{l}{\textbf{Model}}                  & \textbf{mT5D} & \textbf{Gaussion}  & \textbf{Shot} & \textbf{Motion}  & \textbf{Zoom}  & \textbf{Snow}    & \textbf{Bright}   & \textbf{Translate} & \textbf{Rorate} & \textbf{Tilt} & \textbf{Scale} \\ \hline
\multirow{5}{*}{ResNet50}   & Standard         & \best 78.20         &  \best82.00              &  \best79.00         &  \best84.00            &  \best89.00          & \best 80.00            & \best 84.00             &  \best64.00              &  \best 73.00           &  \best80.00         &  \best67.00          \\
                                 & CLIP             & 113.36        & 100.52             & 94.79         & 128.12           & 144.02         & \secbest  118.11           & 144.64            & 97.28              & 102.42          & 124.14        & 79.60          \\
                                 & CLIP-Single      & 117.93        & 106.25             & 99.15         & 132.16           & 149.14         & 121.46           & 152.25            & 100.61             & 106.46          & 129.47        & 82.35          \\
                                 & CLIP-Auto-Single \ours & 115.30        & 103.13             & 97.29         & 129.57           & 145.84         & 120.34           & 146.32            & 98.80              & 104.23          & 126.25        & 81.22          \\
                                 & CLIP-Auto  \ours& \secbest  112.58        &\secbest  99.03              &\secbest  94.11         &\secbest  126.98           &\secbest  142.5          &  118.68           &\secbest  142.34            & \secbest 97.22              & \secbest 102.13          & \secbest 123.32        & \secbest  79.52          \\ \hline
\multirow{5}{*}{ResNet101}  & Standard         & \best 74.37         &\best  80.78              & \best 75.62         & \best 74.82            & \best 81.54          & \best 77.05            &\best  79.30             &\best  62.45              & \best  70.72           & \best 76.21         & \best 65.22          \\
                                 & CLIP             & 102.95        & 88.59              & 84.83         & 113.54           & 130.41         & \secbest 107.79           & 130.73            & 91.34              & 94.19           & 113.95        & 74.17          \\
                                 & CLIP-Single      & 107.45        & 92.91              & 88.14         & 117.57           & 135.26         & 111.7            & 137.86            & 95.48              & 98.38           & 119.82        & 77.36          \\
                                 & CLIP-Auto-Single \ours & 128.32        & 90.70              & 86.31         & 115.18           & 132.54         & 109.41           & 133.19            & 92.95              & 95.79           & 116.17        & 75.23          \\
                                 & CLIP-Auto \ours & \secbest 102.60        & \secbest88.13              &\secbest 84.42         & \secbest113.51           & \secbest129.98         & 107.99           &\secbest 130.05            & \secbest90.82              &\secbest 93.75           & \secbest113.49        & \secbest 73.87          \\ \hline
\multirow{5}{*}{ViT-B/32}   & Standard         & \best 66.58         &  \best42.42              &  \best42.20         &  \best45.85            & \best 56.53          & \best 45.55            &  \best69.09             &  \best 189.21             &  \best 59.54           &  \best 55.92         &  \best 59.53          \\
                                 & CLIP             & 81.19         & 72.78              & 66.85         & 76.38            & 98.42          & 78.51            & 99.52             & 71.46              & 82.40           & 91.56         & 74.04          \\
                                 & CLIP-Single      & 84.68         & 76.22              & 70.58         & 79.60            & 103.31         & 81.50            & 104.26            & 73.82              & 85.56           & 95.67         & 76.29          \\
                                 & CLIP-Auto-Single \ours& 84.13         & 75.10              & 69.52         & 79.76            & 103.05         & 81.25            & 103.51            & 72.92              & 85.09           & 94.85         & 76.23          \\
                                 & CLIP-Auto \ours & \secbest 80.04         & \secbest 70.46              &\secbest  66.04         & \secbest 75.39            & \secbest 97.20          & \secbest 77.84            & \secbest 96.97             & \secbest 70.83              &\secbest  81.85           &\secbest  90.29         & \secbest 73.54          \\ \hline
\multirow{4}{*}{ResNet50x4} & CLIP             & \secbest 98.25         & \secbest 80.76              & \secbest 78.25         & \secbest 114.14           &\secbest 128.89         & \best 109.35           &\secbest  124.89            &\secbest  80.48              & \secbest 88.09           & \secbest 108.25        & \secbest 69.42          \\
                                 & CLIP-Single      & 104.74        & 86.59              & 83.42         & 120.08           & 137.15         & 115.27           & 133.96            & 85.92              & 94.65           & 116.25        & 74.06          \\
                                 & CLIP-Auto-Single \ours & 100.74        & 83.03              & 80.16         & 116.74           & 131.92         & 112.43           & 128.28            & 82.20              & 90.35           & 111.15        & 71.14          \\
                                 & CLIP-Auto \ours &  \best 97.74         & \best 80.19              & \best 77.62         &\best  113.99           & \best 127.88         & \secbest 110.22           &\best  123.88            & \best 79.87              &\best  87.47           & \best 107.30        & \best 69.00          \\ \hline
\end{tabular}
% }
\caption{{\small mT5D.}}
\label{tab:imgnetPmt5d}
\end{subtable}
\caption{{\small Results on ImageNet-P.}}
\end{table}
}

==> tabs/imagenet-P-mt5d.tex <==
\begin{table}[]
\resizebox{0.95\linewidth}{!}{
\begin{tabular}{llccccccccccc}
\hline
\multirow{2}{*}{\textbf{Model}}  & \multicolumn{1}{c}{\textbf{}} & \multicolumn{1}{c|}{\textbf{}}     & \multicolumn{2}{c|}{\textbf{Noise}}                    & \multicolumn{2}{c|}{\textbf{Blur}}                   & \multicolumn{2}{c}{\textbf{Weather}}                 & \multicolumn{4}{c|}{\textbf{Digital}}                                 \\
                                 & \multicolumn{1}{c}{\textbf{}} & \multicolumn{1}{c|}{\textbf{mT5D}} & \textbf{Gaussion} & \multicolumn{1}{c|}{\textbf{Shot}} & \textbf{Motion} & \multicolumn{1}{c|}{\textbf{Zoom}} & \textbf{Snow} & \multicolumn{1}{c|}{\textbf{Bright}} & \textbf{Translate} & \textbf{Rorate} & \textbf{Tilt} & \textbf{Scale} \\ \hline
\multirow{5}{*}{ResNet50}   & Standard         & \best 78.20         &  \best82.00              &  \best79.00         &  \best84.00            &  \best89.00          & \best 80.00            & \best 84.00             &  \best64.00              &  \best 73.00           &  \best80.00         &  \best67.00          \\
                                 & CLIP             & 113.36        & 100.52             & 94.79         & 128.12           & 144.02         & \secbest  118.11           & 144.64            & 97.28              & 102.42          & 124.14        & 79.60          \\
                                 & CLIP-Single      & 117.93        & 106.25             & 99.15         & 132.16           & 149.14         & 121.46           & 152.25            & 100.61             & 106.46          & 129.47        & 82.35          \\
                                 & CLIP-Auto-Single \ours & 115.30        & 103.13             & 97.29         & 129.57           & 145.84         & 120.34           & 146.32            & 98.80              & 104.23          & 126.25        & 81.22          \\
                                 & CLIP-Auto \ours & \secbest  112.58        &\secbest  99.03              &\secbest  94.11         &\secbest  126.98           &\secbest  142.5          &  118.68           &\secbest  142.34            & \secbest 97.22              & \secbest 102.13          & \secbest 123.32        & \secbest  79.52          \\ \hline
\multirow{5}{*}{ResNet101}  & Standard         & \best 74.37         &\best  80.78              & \best 75.62         & \best 74.82            & \best 81.54          & \best 77.05            &\best  79.30             &\best  62.45              & \best  70.72           & \best 76.21         & \best 65.22          \\
                                 & CLIP             & 102.95        & 88.59              & 84.83         & 113.54           & 130.41         & \secbest 107.79           & 130.73            & 91.34              & 94.19           & 113.95        & 74.17          \\
                                 & CLIP-Single      & 107.45        & 92.91              & 88.14         & 117.57           & 135.26         & 111.7            & 137.86            & 95.48              & 98.38           & 119.82        & 77.36          \\
                                 & CLIP-Auto-Single \ours & 128.32        & 90.70              & 86.31         & 115.18           & 132.54         & 109.41           & 133.19            & 92.95              & 95.79           & 116.17        & 75.23          \\
                                 & CLIP-Auto \ours & \secbest 102.60        & \secbest88.13              &\secbest 84.42         & \secbest113.51           & \secbest129.98         & 107.99           &\secbest 130.05            & \secbest90.82              &\secbest 93.75           & \secbest113.49        & \secbest 73.87          \\ \hline
\multirow{5}{*}{ViT-B/32}   & Standard         & \best 66.58         &  \best42.42              &  \best42.20         &  \best45.85            & \best 56.53          & \best 45.55            &  \best69.09             &  \best 189.21             &  \best 59.54           &  \best 55.92         &  \best 59.53          \\
                                 & CLIP             & 81.19         & 72.78              & 66.85         & 76.38            & 98.42          & 78.51            & 99.52             & 71.46              & 82.40           & 91.56         & 74.04          \\
                                 & CLIP-Single      & 84.68         & 76.22              & 70.58         & 79.60            & 103.31         & 81.50            & 104.26            & 73.82              & 85.56           & 95.67         & 76.29          \\
                                 & CLIP-Auto-Single \ours & 84.13         & 75.10              & 69.52         & 79.76            & 103.05         & 81.25            & 103.51            & 72.92              & 85.09           & 94.85         & 76.23          \\
                                 & CLIP-Auto \ours & \secbest 80.04         & \secbest 70.46              &\secbest  66.04         & \secbest 75.39            & \secbest 97.20          & \secbest 77.84            & \secbest 96.97             & \secbest 70.83              &\secbest  81.85           &\secbest  90.29         & \secbest 73.54          \\ \hline
\multirow{4}{*}{ResNet50x4} & CLIP             & \secbest 98.25         & \secbest 80.76              & \secbest 78.25         & \secbest 114.14           &\secbest 128.89         & \best 109.35           &\secbest  124.89            &\secbest  80.48              & \secbest 88.09           & \secbest 108.25        & \secbest 69.42          \\
                                 & CLIP-Single      & 104.74        & 86.59              & 83.42         & 120.08           & 137.15         & 115.27           & 133.96            & 85.92              & 94.65           & 116.25        & 74.06          \\
                                 & CLIP-Auto-Single \ours & 100.74        & 83.03              & 80.16         & 116.74           & 131.92         & 112.43           & 128.28            & 82.20              & 90.35           & 111.15        & 71.14          \\
                                 & CLIP-Auto \ours&  \best 97.74         & \best 80.19              & \best 77.62         &\best  113.99           & \best 127.88         & \secbest 110.22           &\best  123.88            & \best 79.87              &\best  87.47           & \best 107.30        & \best 69.00          \\ \hline
\end{tabular}
}
\caption{{\small mT5D on ImageNet-P.}}
\label{tab:imgnetPmt5d}
\end{table}

==> tabs/imgNetC.tex <==
\begin{table*}[]
\resizebox{\linewidth}{!}{
\begin{tabular}{llccccccccccccccccc}
\hline 
                                 \multirow{2}{*}{\textbf{Model}}  &                  & \multicolumn{1}{l}{}  & \multicolumn{1}{l|}{}                 & \multicolumn{3}{c|}{\textbf{Noise}}                                    & \multicolumn{4}{c|}{\textbf{Blur}}                                                       & \multicolumn{4}{c|}{\textbf{Weather}}                                                & \multicolumn{4}{c}{\textbf{Digital}}                                  \\
                                 &                  & \textbf{Original Acc} & \multicolumn{1}{c|}{\textbf{Avg Acc}} & \textbf{Gauss} & \textbf{Shot} & \multicolumn{1}{c|}{\textbf{Impulse}} & \textbf{Defocus} & \textbf{Glass} & \textbf{Motion} & \multicolumn{1}{c|}{\textbf{Zoom}} & \textbf{Snow} & \textbf{Frost} & \textbf{Fog} & \multicolumn{1}{c|}{\textbf{Bright}} & \textbf{Contrast} & \textbf{Elastic} & \textbf{Pixel} & \textbf{JPEG} \\ \hline
\multirow{5}{*}{ResNet50}   & Standard         & \best 76.13                 & \best 39.17                & \best 29.29          &\best 27.03         & \best 23.81            & \best 38.75            & \best 26.79          & \best 38.67           & \best 36.24         & \best 32.53         & \best 38.14          & \best 45.83        & \best 68.02           & \best39.06             & \best45.25            &\best 44.79          & \best53.41         \\
                                 & CLIP             & 59.85                 & 26.67                & 19.63          & 18.09         & \secbest 12.23            & 26.06            & 14.78          & 25.36           & 23.61         & 22.68         & 26.98          & 38.55        & 50.35           & 32.89             & 28.29            & 28.13          & 32.42         \\
                                 & CLIP-Single      & 57.87                 & 25.34                & 18.77          & 17.28         & 11.73            & 24.90            & 13.86          & 24.07           & 22.47         & 21.37         & 25.05          & 37.19        & 47.76           & 31.69             & 26.83            & 26.78          & 30.35         \\
                                 & CLIP-Auto-Single \ours & 59.86                 & 26.28                & 19.32          & 17.55         & 11.32            & 25.21            & 13.93          & 24.86           & 22.62         & 22.20         & 26.75          & 37.71        & 50.97           & 32.39             & 27.74            & 28.42          & 33.24         \\
                                 & CLIP-Auto \ours        & \secbest 61.78                 & \secbest 27.46                & \secbest 19.93          & \secbest 18.31         & 11.83            &\secbest  27.09            & \secbest 14.90          & \secbest 26.29           & \secbest 24.02         & \secbest 23.26         & \secbest 27.82          &\secbest  39.46        & \secbest 52.38           & \secbest33.95             &\secbest 29.08            &\secbest 29.58          &\secbest 33.97         \\ \hline
\multirow{5}{*}{ResNet101}  & Standard         & \best 77.37                 & \best 44.10                & \best 34.77          & \best 32.63         & \best 29.02            & \best 44.27            & \best32.60           &\best 44.31           & \best40.78         &\best 36.49         &\best 41.73          &\best 49.14        & \best69.85           &\best 42.98             & \best50.11            &\best 53.51          & \best59.30         \\
                                 & CLIP             & 62.32                 & 32.07                & 24.81          & 23.34         & \secbest 19.03            & 31.17            & \secbest 18.77          & 30.14           & 26.90         & \secbest 28.32         & 31.53          & 43.38        & 54.57           & 39.01             & 31.69            & 38.91          & 39.49         \\
                                 & CLIP-Single      & 60.65                 & 30.48                & 23.93          & 22.30         & 18.03            & 30.06            & 17.67          & 29.17           & 26.21         & 26.35         & 29.12          & 41.16        & 51.99           & 37.33             & 29.98            & 36.77          & 37.09         \\
                                 & CLIP-Auto-Single \ours & 62.86                 & 31.98                & 24.88          & 23.20         & 18.45            & 31.46            & 18.57          & 30.69           & 27.34         & 27.88         & 31.06          & 43.03        & 54.50           & 39.24             &  31.61            & 38.63          & 39.11         \\
                                 & CLIP-Auto \ours        &\secbest 63.83                 & \secbest32.57                &\secbest 25.31          & \secbest23.60         & 18.93            & \secbest31.81            & 18.75          & \secbest30.85           & \secbest27.51         & 28.20         & \secbest31.80          & \secbest44.14        & \secbest55.68           & \secbest39.89             &\secbest 32.11            &\secbest 39.44          & \secbest 40.46         \\ \hline
                                 
\multirow{5}{*}{ViT-B/16}   & Standard         & \best 84.20                & 60.12 & 54.11 & 52.74 & 52.14 & 54.28 & 51.4 & 62.84 & 55.21 & 60.48 & 59.03 & 61.48 & 78.18 & 55.7 & 63.15 & 71.46 & 69.63         \\
                                 & CLIP             & 68.43                 & 43.87 & 39.48 & 37.82 & 35.05 & 42.03 & \secbest 33.22 & 44.75 & 36.60 & 43.52 & 42.72 & 51.53 & 62.33 & 47.92 & 41.27 & 49.76 & 50.01         \\
                                 & CLIP-Sinlge      & 66.94                 &42.13 & 37.81 & 36.03 & 33.28 & 40.61 & 31.97 & 42.99 & 34.84 & 41.82 & 40.64 & 50.13 & 60.04 & 46.64 & 39.78 & 47.55 & 47.86          \\
                                 & CLIP-Auto-Single \ours & 68.61                 & 43.21 & 39.18 & 37.53 & 34.09 & 41.65 & 32.23 & 44.32 & 36.05 & 43.02 & 41.82 & 50.28 & 62.29 & 46.15 & 40.18 & 49.12 & 50.28     \\
                                 & CLIP-Auto  \ours       & \secbest69.51                 &\secbest  44.19 &\secbest 39.79 & \secbest38.09 &\secbest 35.08 & \secbest42.44 & 33.17 & \secbest45.08 &\secbest 36.83 & \secbest43.93 & \secbest42.94 &\secbest 51.76 & \secbest63.17 &\secbest 48.09 &\secbest 41.30 & \secbest50.24 & \secbest50.91       \\ \hline
                                 
                                 
                                 
                                
                                

\multirow{5}{*}{ViT-B/32}   & Standard         & \best 78.73                 & \best 50.79                & \best 44.05          &\best  41.40         &\best 41.30            &\best 48.59            & \best45.81          &\best 54.48           & \best43.20         & \best31.50         &\best 38.99          & \best56.81        & \best67.77           & \best59.72             & \best57.45            & \best66.59          & \best64.13         \\
                                 & CLIP             & 63.40                 & 40.31                & 37.21          & 35.36         & 33.65            & 40.34            & 29.18          & 41.17           & 32.13         & 34.29         & 37.13          & 46.52        & 57.62           & 45.22             & 40.96            & 47.26          & 46.60         \\
                                 & CLIP-Sinlge      & 61.82                 & 39.18                & 36.17          & 34.18         & 32.55            & 39.12            & 28.29          & 39.99           & 30.79         & 33.47         & 35.95          & 45.32        & 56.28           & 44.25             & 39.75            & 46.11          & 45.47         \\
                                 & CLIP-Auto-Single \ours & 63.13                 & 39.42                & 36.01          & 34.02         & 32.21            & 39.25            & 27.98          & 40.68           & 31.50         & 33.59         & 36.09          & 45.72        & 57.20           & 43.59             & 40.65            & 46.61          & 46.15         \\
                                 & CLIP-Auto  \ours       & \secbest65.16                 &\secbest 41.04                &\secbest 37.77          & \secbest35.69         & \secbest33.95            & \secbest41.12            & \secbest29.44          &\secbest 42.19           &\secbest 32.65         &\secbest 34.65         & \secbest37.43          & \secbest47.27        & \secbest59.14           & \secbest46.15             &\secbest 41.97            & \secbest48.35          & \secbest47.81         \\ \hline

                                 
                                 
                                 


\multirow{4}{*}{ResNet50x4} & CLIP             &\secbest 66.28                 & \best34.43                & \best27.76          & \best26.57         & \best23.59            &\best31.36            & \best18.70           &\best 31.67           & \best28.34         & \best30.77         &\best 34.39          &\best 45.72        & \secbest57.81           &\best 39.80             & \best32.57            &\secbest 42.40           & 44.94         \\
                                 & CLIP-Sinlge      & 64.12                 & 32.44                & 26.31        & 24.72         & 21.96            & 28.54            & 17.14          & 28.87           & 25.95         &  28.40         & 31.49          & 42.18        & 54.34           & 36.96             & 30.14            & 38.41          & 41.35         \\
                                 & CLIP-Auto-Single \ours & 65.45                 &\secbest 33.98                & 26.83          & 25.81         & 22.51            & 30.58            & \secbest 18.41          & \secbest 31.61           & \secbest 28.40         & \secbest 30.63         & 33.53          & 44.43        & 57.18           & 39.46             & 31.90            & \best 42.89          & \best 45.58         \\
                                 & CLIP-Auto  \ours       & \best66.48                 &\secbest 33.98                & \secbest27.05          &\secbest 25.82         &\secbest 22.84            &\secbest 30.60            & 18.04          &  30.85           & 27.75         & 30.44         & \secbest33.98          & \secbest45.15        &\best 57.83           & \secbest39.78             & \secbest32.21            &  42.17          & \secbest45.23         \\ \hline
                                 
\multirow{4}{*}{ResNet50x16} & CLIP             &\secbest 70.67                 & \best 41.39 & \best 38.22 & \best 37.16 & \best 35.15 & \best 36.60 & \best 23.49 & \best 38.34 & \best 34.08 & \best 38.08 & \best 39.33 & \best 50.88 & \best 62.37 & \best 46.23 & \best 37.68 & \secbest49.67 &\secbest 53.63         \\
                                 & CLIP-Sinlge      & 67.57                & 38.02 & 35.17 & 34.20 & 31.76 & 33.57 & 21.56 & 35.19 & 31.40 & 34.78 & 35.97 & 46.78 & 58.46 & 42.84 & 34.56 & 44.40 & 49.73     \\
                                 
                                 & CLIP-Auto-Single \ours & 67.17                &38.07 & 34.88 & 33.71 & 31.97 & 33.55 & 21.00 & 34.59 & 30.63 & 34.38 & 36.19 & 47.59 & 58.69 & 43.00 & 34.77 & 45.97 & 50.14        \\
                                 
                                 & CLIP-Auto  \ours       & \best 70.81                & \secbest40.93 & \secbest37.63 &\secbest 36.34 &\secbest 34.68 & \secbest36.22 & \secbest22.55 & \secbest37.55 & \secbest32.95 & \secbest37.22 & \secbest38.93 & \secbest50.56 & \secbest62.42 & \secbest46.00 & \secbest37.13 & \best 50.05 & \best 53.66  \\ \hline
                                 
                                 
                                 
\end{tabular}

}
\caption{{ Individual top-1 accuracy scores on all the corruption types of ImageNet-C. ``Original Acc'' refers to the accuracy of the clean ImageNet validation set. ``Avg Acc'' denotes the average accuracy of 15 common corruptions. CLIP reduces the average robustness of ImageNet-C, as ImageNet-C overlaps less with the pre-training set of CLIP. Note that there is no corresponding standard ResNet50x4 model available.}}
\label{tab:inc}
\end{table*}




==> tabs/natural.tex <==
\begin{table*}[]
\resizebox{\linewidth}{!}{
\begin{tabular}{llcccccccc}
\hline
\multicolumn{2}{l}{\textbf{Model}}               & \textbf{ImageNet} & \textbf{ImageNetV2} & \textbf{ImageNet-R} & \textbf{ObjectNet} & \textbf{ImageNet-Sketch} & \textbf{ImageNet-A} & \textbf{Youtube-BB} & \textbf{ImageNet-Vid} \\ \hline
\multirow{5}{*}{ResNet50}   & Standard           & \best 76.13                              & \best 62.70                                & 35.05                                & 35.77                               & 22.20                                 & 0.81                                 & 50.10                                & 60.14                                  \\
                            & CLIP               & 59.85                              & 52.64                                & \best 60.51                                & \best 39.82                               & \secbest 35.46                                & \secbest 22.75                                & \best 56.69                                & \best 64.92                                  \\
                            & CLIP-Single        & 57.87                              & 51.09                                & 56.12                                & \secbest39.48                               & 33.24                                & 21.77                                & 55.33                                & 63.70                                  \\
                            & CLIP-Auto-Single \ours   & 59.86                              & 52.59                                & 57.56                                & 35.85                               & 34.01                                & 20.61                                & 55.52                                & 63.53                                  \\
                            & CLIP-Auto \ours & \secbest 61.78                              &\secbest 54.53                                & \secbest 60.48                                & 39.21                               & \best35.48                                & \best 23.81                                & \secbest56.68                                &\secbest 64.61                                  \\ \hline
\multirow{5}{*}{ResNet101}  & Standard           & \best 77.37                              & \best 65.04                                & 38.45                                & 38.41                               & 25.86                                & 4.79                                 & 53.10                                & 62.80                                  \\
                            & CLIP               & 62.32                              & 56.08                                & \best 68.01                                & 44.17                               & \best 41.09                                & \secbest 29.44                                & \secbest 61.75                                & \secbest 71.28                                  \\
                            & CLIP-Single        & 60.65                              & 54.31                                &  63.83                                & 43.56                               & 38.02                                & 27.95                                & 57.39                                & 68.66                                  \\
                            & CLIP-Auto-Single \ours   & 62.86                              & 55.84                                & 66.74                                & \secbest 44.49                               & 40.30                                & 28.97                                & 60.82                                & 70.78                                  \\
                            & CLIP-Auto \ours & \secbest 63.83                              & \secbest 56.95                                &\secbest 67.37                                & \best 45.01                               & \secbest 40.89                                & \best 30.36                                & \best 62.11                                & \best 71.64                                  \\ \hline
\multirow{5}{*}{ViT-B/32}   & Standard           &  \best 78.73                              & \best 71.16                                &  44.69                                & \best 43.76                               & 32.55                                &\best 33.64                                & \best 63.62                                & \best 77.72                                  \\
                            & CLIP               & 63.40                              & 55.73                                & \best 69.29                                & \secbest 43.60                               & \best 42.42                                & 31.35                                & 60.98                                & 74.03                                  \\
                            & CLIP-Single       & 61.82                              & 54.67                                & 66.61                                & 43.56                               & 40.86                                & 30.20                                & 60.82                                & 74.12                                  \\
                            & CLIP-Auto-Single \ours   & 63.13                              & 56.05                                & 66.18                                & 42.16                               & 40.28                                & 30.75                                & 59.14                                & 73.40                                  \\
                            & CLIP-Auto \ours & \secbest 65.16                              & \secbest 57.51                                & \secbest 68.10                                & 43.16                               & \secbest 42.15                                & \secbest 32.21                                & \secbest 61.01                                & \secbest 74.80                                  \\ \hline
\multirow{5}{*}{ViT-B/16}   & Standard           &  \best 84.20                              & \best 74.13 &	50.89 &	51.12	& 38.10 &	\best 50.64 &	\best 64.76 & \best 81.79                                   \\
                            & CLIP               & 66.94                           & 62.52 & \best	77.82 &	\best 53.45 &	\best 48.47 &	49.39 &	\secbest 64.07    & 80.26                        \\
                            & CLIP-Single       & 66.94                              & 60.88 &	74.10	& 53.03	 & 46.42 &	47.24 &	63.57 & \secbest 81.34                            \\
                            & CLIP-Auto-Single \ours   & 68.61                              & 61.96	& 75.86 & 	52.11 &	47.50 &	49.11	 & 61.14    & 77.91                              \\
                            & CLIP-Auto \ours & \secbest 69.51                             & \secbest 63.11	& \secbest 76.83	 & \secbest 53.08 & 	\secbest 48.43 &	\secbest 49.56	& 63.28	 & 79.76                         \\ \hline
\multirow{4}{*}{ResNet50x4} & CLIP               & \secbest 66.28                              &\secbest 59.34                                & \best 72.63                                & \secbest 49.97                               & \best 44.75                                & \best 41.53                                & \secbest 59.53                                & \best 72.50                                  \\
                            & CLIP-Single        & 64.12                              & 57.33                                & 68.01                                & 49.50                               & 41.57                                & 38.41                                & 58.31                                & 69.79                                  \\
                            & CLIP-Auto-Single \ours  & 65.45                              & 58.11                                & 70.67                                & 47.57                               & 44.05                                & 39.51                                & 56.97                                & \secbest 72.41                                  \\
                            & CLIP-Auto \ours & \best 66.48                              & \best 59.75                                &\secbest 71.33                                & \best 50.36                               & \secbest 44.55                                & \secbest 40.95                                & \best 59.75                                & 72.14                                  \\ \hline
                            
                            
\multirow{4}{*}{ResNet50x16} & CLIP               & \secbest 70.67                              & \best  64.14 &	\best  79.18 &	\secbest 58.86	& \best 50.66 & 	\best 56.41 & 	\best 62.96 &	\best 78.45 \\
                            & CLIP-Single        & 67.57                             & 60.53 &	 74.69 & 	57.57 &	47.48 &	51.61 &	59.63 &	76.29                                \\
                            & CLIP-Auto-Single \ours  & 67.17                              & 60.65 &	75.33 &	52.75 &	46.73 &	53.51 &	55.76 &	71.96    \\
                            & CLIP-Auto \ours & \best 70.81                            & \secbest 63.90 &	\secbest 78.33 &	\best  59.04 &	\secbest 49.62 &	\secbest 55.93 &	\secbest 61.97 &	\secbest 78.04                               \\ \hline
\end{tabular}%
}
\vspace{-0.05in}
    \caption{{\small Model accuracies on ImageNet and seven natural distribution shifts.}}
        \label{table:natural}
\end{table*}

\comm{
\begin{table*}[]
\resizebox{\linewidth}{!}{
\begin{tabular}{llcccccccc}
\hline
\multicolumn{2}{l}{\textbf{Model}}               & \textbf{ImageNet} & \textbf{ImageNetV2} & \textbf{ImageNet-R} & \textbf{ObjectNet} & \textbf{ImageNet-S} & \textbf{ImageNet-A} & \textbf{Youtube-BB} & \textbf{ImageNet-Vid} \\ \hline
\multirow{5}{*}{ResNet50}   & Standard           & 76.13             & 62.70               & 35.05               & 35.77              & 22.20                & 0.81                & 50.10               & 60.14                 \\
                            & CLIP               & 57.87             & 51.09               & 56.12               & 39.48              & 33.24               & 21.77               & 55.33               & 63.70                 \\
                            & CLIP-Ensemble      & 59.85             & 52.64               & \best 60.51               & \best 39.82              & \secbest 35.46               & \secbest 22.75               & \best 56.69               & 64.92                 \\
                            & CLIP-Auto-Single   & 59.86             & 52.59               & 57.56               & 35.85              & 34.01               & 20.61               & 55.52               & 63.53                 \\
                            & CLIP-Auto-Ensemble & 61.78             & 54.53               & \secbest 60.48               & 39.21              & 35.48               & 23.81               & \secbest 56.68               & 64.61                 \\ \hline
\multirow{5}{*}{ResNet101}  & Standard           & 77.37             & 65.04               & 38.45               & 38.41              & 25.86               & 4.79                & 53.10               & 62.80                 \\
                            & CLIP               & 60.65             & 54.31               & 63.83               & 43.56              & 38.02               & 27.95               & 57.39               & 68.66                 \\
                            & CLIP-Ensemble      & 62.32             & 56.08               & 68.01               & 44.17              & 41.09               & 29.44               & \secbest 61.75               & 71.28                 \\
                            & CLIP-Auto-Single   & 62.86             & 55.84               & 66.74               & 44.49              & 40.30               & 28.97               & 60.82               & 70.78                 \\
                            & CLIP-Auto-Ensemble & 63.83             & 56.95               & 67.37               & 45.01              & 40.89               & 30.36               & 62.11               & \best 71.64                 \\ \hline
\multirow{5}{*}{ViT-B/32}   & Standard           & 78.73             & 67.42               & 39.40               & \best 43.76              & 19.35               & 24.17               & 63.62               & \best 77.72                 \\
                            & CLIP               & 61.82             & 54.67               & 66.61               & 43.56              & 40.86               & 30.20               & 60.82               & 74.12                 \\
                            & CLIP-Ensemble      & 63.40             & 55.73               & 69.29               & 43.60              & 42.42               & 31.35               & 60.98               & 74.03                 \\
                            & CLIP-Auto-Single   & 63.13             & 56.05               & 66.18               & 42.16              & 40.28               & 30.75               & 59.14               & 73.40                 \\
                            & CLIP-Auto-Ensemble & 65.16             & 57.51               & 68.10               & 43.16              & 42.15               & 32.21               & 61.01               & \secbest 74.80                 \\ \hline
\multirow{4}{*}{ResNet50x4} & CLIP               & 64.12             & 57.33               & 68.01               & 49.50              & 41.57               & 38.41               & 58.31               & 69.79                 \\
                            & CLIP-Ensemble      & 66.28             & 59.34               & 72.63               & \secbest 49.97              & 44.75               & 41.53               & 59.53               & 72.50                 \\
                            & CLIP-Auto-Single   & 65.45             & 58.11               & 70.67               & 47.57              & 44.05               & 39.51               & 56.97               & \secbest 72.41                 \\
                            & CLIP-Auto-Ensemble & 66.48             & 59.75               & 71.33               & 50.36              & 44.55               & 40.95               & 59.75               & 72.14                 \\ \hline
\end{tabular}%
}

    \caption{\focus{\small Model accuracies on natural distribution shifts.}}
        \label{table:natural}
\end{table*}
}

\comm{
\begin{table*}[]
\resizebox{0.95\linewidth}{!}{
\begin{tabular}{|c|l|l|l|l|l|l|l|l|l|}
\hline
\multicolumn{2}{|l|}{Model}                      & ImageNet & ImageNetv2 & ImageNet-R     & ObjectNet      & ImageNet-S & ImageNet-A & Youtube-BB     & ImageNet-Vid   \\ \hline
\multicolumn{2}{|l|}{ResNet50}                   & 76.13    & 62.70      & 35.05          & 35.77          & 22.20       & 0.81       & 50.10          & 60.14          \\ \hline
\multicolumn{2}{|l|}{ResNet101}                  & 77.37    & 65.04      & 38.45          & 38.41          & 25.86      & 4.79       & 53.10          & 62.80          \\ \hline
\multicolumn{2}{|l|}{ViT-B/32}                   & 78.73    & 67.42      & 39.40          & 43.76          & 19.35      & 24.17      & 63.62          & 77.72          \\ \hline
\multirow{4}{*}{CLIP-ResNet50}   & Original      & 57.87    & 51.09      & 56.12          & 39.48          & 33.24      & 21.77      & 55.33          & 63.70          \\ \cline{2-10} 
                                 & Single Prompt & 59.86    & 52.59      & \textbf{57.56} & \textbf{35.85} & 34.01      & 20.61      & \textbf{55.52} & \textbf{63.53} \\ \cline{2-10} 
                                 & Manual Prompt & 59.85    & 52.64      & \best 60.51          & \best 39.82          & 35.46      & 22.75      & 56.69          & 64.92          \\ \cline{2-10} 
                                 & LEAP          & 61.78    & 54.53      & 60.48          & 39.21          & 35.48      & \best 23.81      & 56.68          & 64.61          \\ \hline
\multirow{4}{*}{CLIP-ResNet101}  & Original      & 60.65    & 54.31      & 63.83          & 43.56          & 38.02      & 27.95      & 57.39          & 68.66          \\ \cline{2-10} 
                                 & Single Prompt & 62.86    & 55.84      & 66.74          & 44.49          & 40.30      & 28.97      & 60.82          & 70.78          \\ \cline{2-10} 
                                 & Manual Prompt & 62.32    & 56.08      & 68.01          & 44.17          & 41.09      & 29.44      & 61.75          & \secbest 71.28          \\ \cline{2-10} 
                                 & LEAP          & 63.83    & 56.95      & 67.37          & 45.01          & 40.89      & 30.36      & 62.11          & 71.64          \\ \hline
\multirow{4}{*}{CLIP-ResNet50x4} & Original      & 64.12    & 57.33      & 68.01          & 49.50          & 41.57      & 38.41      & 58.31          & 69.79          \\ \cline{2-10} 
                                 & Single Prompt & 65.45    & 58.11      & 70.67          & 47.57          & 44.05      & 39.51      & 56.97          & 72.41          \\ \cline{2-10} 
                                 & Manual Prompt & 66.28    & 59.34      & 72.63          & 49.97          & 44.75      & 41.53      & 59.53          & 72.50          \\ \cline{2-10} 
                                 & LEAP          & 66.48    & 59.75      & 71.33          & 50.36          & 44.55      & 40.95      & 59.75          & 72.14          \\ \hline
\multirow{4}{*}{CLIP-ViT-B/32}   & Original      & 61.82    & 54.67      & 66.61          & 43.56          & 40.86      & 30.20      & 60.82          & 74.12          \\ \cline{2-10} 
                                 & Single Prompt & 63.13    & 56.05      & 66.18          & 42.16          & 40.28      & 30.75      & 59.14          & 73.40          \\ \cline{2-10} 
                                 & Manual Prompt & 63.40    & 55.73      & 69.29          & 43.60          & 42.42      & 31.35      & 60.98          & 74.03          \\ \cline{2-10} 
                                 & LEAP          & 65.16    & 57.51      & 68.10          & 43.16          & 42.15      & 32.21      & 61.01          & 74.80          \\ \hline
\end{tabular}


}

    \caption{\focus{\small Model accuracies on natural distribution shifts.}}
        \label{table:natural}
\end{table*}
}



==> tabs/typo.tex <==
\begin{table*}[]
\resizebox{0.95\linewidth}{!}{
\begin{tabular}{llcc}
\toprule
\multicolumn{2}{l}{\textbf{Model}  }                    & \textbf{CIFAR-10-T (Success rate / Accuracy)} & \textbf{ImageNet-T (Success rate / Accuracy) }\\ \midrule
\multirow{5}{*}{ResNet50}   & Standard         & \best  8.16 / 13.90                      & \best  0.03 / 68.66                       \\
                            & CLIP             & 99.40 / 0.22                      & 40.42 / 22.61                      \\
                            & CLIP-Single      & 99.38 / 0.25                      & 40.08 / 21.02                      \\
                            & CLIP-Auto-Single \ours & \secbest 99.20 / 3.50                      & \secbest 32.29 / 25.08                      \\
                            & CLIP-Auto  \ours      & 99.46 / 0.18                      & 44.86 / 21.50                      \\ \midrule
\multirow{5}{*}{ResNet101}  & Standard         & \best 6.49 / 27.03                      & \best 0.03 / 69.70                       \\
                            & CLIP             & \secbest 97.97 / 1.61                      & \secbest 37.76 / 25.25                      \\
                            & CLIP-Single      & 98.16 / 1.37                      & 39.06 / 22.51                      \\
                            & CLIP-Auto-Single \ours & 98.57 / 1.02                      & 45.09 / 22.12                      \\
                            & CLIP-Auto \ours        & 98.07 / 1.45                      & 42.47 / 23.93                      \\ \midrule

\multirow{5}{*}{ViT-B/16}   & Standard         & \best 7.04 / 35.67                    &\best  0.02 / 80.05                      \\
                            & CLIP             & 89.84 / 9.51                     & 25.07 / 45.59                      \\
                            & CLIP-Single      & 90.76 / 8.64                     & 26.99 / 42.69                    \\
                            & CLIP-Auto-Single \ours & \secbest 86.24 / 12.08                     & \secbest 22.28 / 46.69                       \\
                            & CLIP-Auto   \ours     & 90.54 / 8.79                    &  25.14 / 45.99                     \\ \midrule
                            
                            
                            
\multirow{5}{*}{ViT-B/32}   & Standard         & \best 3.73 / 65.12                      &\best  0.02 / 75.03                       \\
                            & CLIP             & 77.47 / 17.08                     & 13.07 / 45.06                      \\
                            & CLIP-Single      & 80.09 / 14.69                     & 15.13 / 42.52                      \\
                            & CLIP-Auto-Single \ours & \secbest 72.03 / 19.33                     & 9.52 / 46.99                       \\
                            & CLIP-Auto   \ours     & 75.24 / 17.67                     & \secbest 12.64 / 47.01                      \\ \midrule


\multirow{4}{*}{ResNet50x4} & CLIP             & 98.75 / 1.06                      & \best 44.21 / 27.14                      \\
                            & CLIP-Single      &\secbest  98.28 / 1.50                      & 49.02 / 22.84                      \\
                            & CLIP-Auto-Single \ours& \best 95.64 / 2.77                      & \secbest 47.41 / 25.69                      \\
                            & CLIP-Auto  \ours      & 99.13 / 0.72                      & 48.28 / 24.90                      \\ \midrule


\multirow{4}{*}{ResNet50x16} & CLIP             & 97.85 / 2.07                     & \best 50.22 / 27.99                     \\
                            & CLIP-Single      &\best  95.53 / 3.99                      & 52.37 / 23.62                     \\
                            & CLIP-Auto-Single \ours& \secbest 96.13 / 3.60                      & \secbest 55.30 / 23.34                       \\
                            & CLIP-Auto  \ours      & 97.59 / 2.30                     &  \secbest 52.29 / 26.80                   \\ \bottomrule
\end{tabular}
}
    \caption{{ Model accuracies and success rates under typographic attacks on ImageNet-T and CIFAR-10-T. We highlight the results based on the accuracy. CLIP causes a significant robustness drop compared to the corresponding standard models. This again implies the importance of studying the impact of both data and model on robustness.}}
    \label{tab:typo}
    
\end{table*}
